Revisiting Efficient Multi-Step Nonlinearity Compensation with Machine Learning: An Experimental Demonstration

Efficient nonlinearity compensation in fiber-optic communication systems is considered a key element to go beyond the "capacity crunch''. One guiding principle for previous work on the design of practical nonlinearity compensation schemes is that fewer steps lead to better systems. In this paper, we challenge this assumption and show how to carefully design multi-step approaches that provide better performance--complexity trade-offs than their few-step counterparts. We consider the recently proposed learned digital backpropagation (LDBP) approach, where the linear steps in the split-step method are re-interpreted as general linear functions, similar to the weight matrices in a deep neural network. Our main contribution lies in an experimental demonstration of this approach for a 25 Gbaud single-channel optical transmission system. It is shown how LDBP can be integrated into a coherent receiver DSP chain and successfully trained in the presence of various hardware impairments. Our results show that LDBP with limited complexity can achieve better performance than standard DBP by using very short, but jointly optimized, finite-impulse response filters in each step. This paper also provides an overview of recently proposed extensions of LDBP and we comment on potentially interesting avenues for future work.

==> appendices/app1.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Detailed Explanation of Something} \label{app:app1}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> sections/dbpwithpd.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%
%\section{Digital Backpropagation} 
%\label{sc:dbppdl}
%%%%%%%%%%%%%%%%%%%%%%%%

Standard DBP considers chromatic dispersion, attenuation, and nonlinearity compensation only. Other effects such as PMD and PDL have a statistical unpredictable behaviour. Therefore, these effects are usually not compensated in DBP, unless in some specifically proposed algorithms []. In this section, we describe the standard DBP and its numerical implementation.


% DBP for an optical fiber is obtained by inverting the distance direction in the previous forward propagation equations. This direction change is accomplished by considering $N_B$ inversely ordered points $z_l$ in a fiber span of length $L$, $1\le l \le N_B$, where $z_0=L$ and $z_{N_B}=0$. 


% Usually, $N_B<<N_s$ to reduce the complexity of the DBP algorithm. The definition of $\Delta z_k$ is analogous to the previous section, given by $\Delta z_k = z_{k}-z_{k-1}$, $1 \le k \le N_B$. Due to the different order of the points $z_l$, $\Delta z_k$ now assumes negative values.


% In a numerical framework, the signal $\bE$ is represented by $N_t$ samples in time domain, with sampling period $T$. We will represent this sample signal by a vector $\bu$ of dimension $N_t\times 2$, as a function of distance $z$. By using this notation, the field $\bu(z_k)$ at the distance $z_k$ is given by
% \begin{align}
%     \bu(z_k) &\triangleq \bu(\cdot,z_k) \notag \\ &= \left[\begin{array}{cccc} \bu(T,z_k) & \bu(2T,z_k) & \cdots  & \bu(N_t T,z_k) \end{array} \right]' \notag \\
%     &= \left[ \begin{array}{cccc}
%         u_x(T,z_k) & u_x(2T,z_k)& \cdots & u_x(N_t T,z_k)  \\
%         u_y(T,z_k) & u_y(2T,z_k)& \cdots & u_y(N_t T,z_k)  
%     \end{array}\right]',
% \end{align}
% where $u_x,u_y \in \mathbb{C}$ represent the  time samples of $\bu$ in the $x-$ and $y-$polarizations, respectively. 



%To evaluate $\bu$ in a nonzero distance, the most used method is the SSFM, which is represented in Fig.~\ref{}. As shown in that figure, the method consists in dividing a fiber span of length $L$ into $N_z$ small segments of length $\Delta z_k$, $1\le k \le N_z$, $\sum_{r=1}^{N_z}\Delta z_{r}=L$. We will denote $z_k =\sum_{r=1}^{k}\Delta z_{r}$, with $z_0 = 0$. At a certain distance $z_{k-1}$, the propagation effects present in $\eqref{eq:mnkvpmd}$ are individually applied to $u(z_{k-1})$, resulting in the field $u$ at the new distance $z_k$, given by $u(z_k)$. To simplify the notation, we denote $\bus$ and $\but$ the field $\bu$ before and after applying each of these fiber effects. The expressions for $\but$ are derived based on the solution simplified differential equations that consider each effect solely. The details of this procedure are given in the following sections.






%%%%%%%%





%In the SSFM, we consider $z=z_k$ and $z'=z_{k-1}$. Thus, the equivalents of \eqref{eq:attsolsimp}, \eqref{eq:attsolsimplump}, and \eqref{eq:attpdl} in the numerical domain are, respectively,
% \begin{align}\label{eq:attnum1}
%     \but(z_{k-1}) &= e^{-\frac{1}{2}\int_{z_{k-1}}^{z_k} \alpha(u)\text{d}u} \bus(z_{k-1}), \\ \label{eq:attnum2}
%      \but(z_{k-1}) &= e^{-\frac{1}{2}\alpha\Delta z_k} \bus(z_{k-1}), \\ 
%      \label{eq:attnum3}
%      \but(z_{k-1}) &= g\bM \bus(z_{k-1}).
% \end{align}
% We chose to write $\but(z_{k-1})$ in the left-hand side of \eqref{eq:attnum1}, \eqref{eq:attnum2}, and \eqref{eq:attnum3} to emphasize that $\bu(z_k)$ is only obtained after applying to $\bus(z_{k-1})$ all the effects present in \eqref{eq:mnkvpmd}.



%%%%%%%%%%%%%%%%%%%%%
% To implement \eqref{eq:dispFsol} numerically, the standard approach is to apply a fast Fourier transform (FFT) to the field $\bu$, on each polarization separately. This operation will be denoted, without loss of generality, by a discrete Fourier transform (DFT) matrix $\bF \in \mathbb{C}^{N_t\times N_t}$ to simplify the notation and the mathematical operations. The inverse FFT (IFFT) will be represented by the inverse DFT (IDFT) matrix $\bF^{-1}$. With this representation, the field $\bu$ at distance $z_{k-1}$ after applying the chromatic dispersion effect is given by
% \begin{equation}
%   \bu(z_{k-1}) \bF \text{diag}(H_1,H_2, \cdots , H_{N_t}) \bF^{-1},
% \end{equation}
% where $H_i = -j \frac{\beta_2}{2} \omega_i^2 \Delta z_k $, $\omega_i = 2 \pi f_i$ is the $i$-th DFT angular frequency.

==> sections/experimentalsetup.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%
\section{Experimental Setup and Receiver DSP} 
\label{sc:expset}
%%%%%%%%%%%%%%%%%%%%%%%%

In this paper, we conduct an experimental validation of LDBP focusing on single-channel DBP of a polarization-multiplexed $25$ Gbaud signal over $1500$ km of SSMF. This section describes the recirculating loop setup used to obtain the experimental data and the corresponding DSP chain used to process that experimental data.

\subsection{Experimental Recirculating Loop Setup}
\begin{figure*}
    \centering
    \input{tikz/dspchain.tikz}
    \caption{Representation of the DSP chain applied to the digitized fiber output detected by the coherent receiver and analog-to-digital converter as shown in Fig.~\ref{fig:experimental_setup}.}% F-E: Front-End; F.O.: Frequency Offset; Ph.-N. Comp.: Phase Noise Compensation.}
    \label{fig:dspchain}
\end{figure*}

A schematic of the experimental transmission  setup is depicted in Fig~\ref{fig:experimental_setup}. Sequences are generated offline using pseudorandom bit sequences (PRBS) and contain \(2^{16}\) symbols. These are pulse-shaped using a root-raised cosine (RRC) filter with 1\% roll-off, digitally pre-compensated for transmitter bandwidth limitations and uploaded to a 100-GSa/s digital-to-analog converter (DAC). The \(193.4\) THz carrier is generated by an external cavity laser (ECL), modulated by a dual-polarization IQ-modulator (DP-IQM) and amplified using an erbium doped fiber amplifier (EDFA). Using acousto-optic modulators (AOMs), the optical signal is circulated in a recirculating loop consisting of a loop-synchronised polarization scrambler (LSPS), a 75-km span of SSMF, an EDFA and an optical tunable filter (OTF) for gain equalization. At the receiver side, the optical signal is amplified with an EDFA, filtered using a wavelength selective switch (WSS) and received by an intradyne coherent receiver consisting of a local oscillator (LO), 90-degree hybrid and 4 balanced photodiodes. The resulting electrical signal is digitized by an 80-GSa/s real-time oscilloscope and receiver DSP is performed offline, as described in the next section.

%which consists of front-end compensation and frequency-offset compensation.


\subsection{Receiver DSP Blocks}
\label{sc:dsp}


The receiver DSP used in the experimental setup consists of seven blocks, which are applied sequentially. These blocks are represented in Fig.~\ref{fig:dspchain} and described in the following.


\begin{enumerate}
    \item \textit{Receiver Optical Front-End IQ Compensation:}\\
    Orthonormalization using blind moment estimation. This compensates the gain imbalance and offset angle between the in-phase and quadrature components.
    \item \textit{Resampling:}\\
    Rational resampling to 2 samples per symbol.
     \item \textit{Frequency-Offset Compensation:}\\
    Estimate and correct for frequency offset between transmitter and local oscillator laser.
    \item \textit{Static Equalization:}\\
    Here, we consider three cases: (i) chromatic dispersion compensation (CDC), (ii) conventional DBP, and (iii) LDBP.
    % \item \textit{Matched filter:}\\
    % Ideal RRC filter with $1\%$ roll-off, implemented in frequency domain. 
    \item \textit{Adaptive Equalization and phase-noise compensation:}\\
    MIMO equalizer trained with standard mean-squared error (MSE) metric. The MIMO equalizer is used to recover the signal state of polarization and partially compensate for other impairments, such as PMD. Inside the update-loop of the equalizer, blind phase search (BPS) using the known transmitted symbols removes phase noise.
    \item \textit{Downsampling and Time Alignment:}\\
    The signal is downsampled to 1 sample per symbol and aligned with the transmitted sequence.
    % \item \textit{Phase-Noise Compensation:}\\
    \item \textit{Effective SNR Estimation:}\\
    Finally, we determine the effective SNR which is used as the main figure of merit in this paper. 
\end{enumerate}

% \subsubsection{Receiver Optical Front-End IQ Compensation}
% Orthonormalization of the in-phase and quadrature components using blind moment estimation.
% \subsubsection{Frequency-Offset Compensation}
% Estimate and correct for frequency offset between transmitter and local oscillator laser.
% \subsubsection{Resampling}
% Rational resampling to 2 samples per symbol.
% \subsubsection{Static Equalization} Here, we consider three cases: (i)  chromatic dispersion compensation (CDC), (ii) conventional DBP, and (iii) LDBP. 
% \subsubsection{Matched filter}
% \subsubsection{Adaptive Equalization} MIMO equalizer trained with standard SGD
% \subsubsection{Downsampling and Time Alignment}
% \subsubsection{Phase-Noise Compensation}
% \subsubsection{Effective SNR Estimation} Finally, we measure the effective SNR which is used as the main figure of merit in this paper. 

% \begin{center}
% \begin{tabular}{c|c|c|c}
% \hline
%     \multicolumn{4}{c}{Possible Experimental Setups}  \\
%     \hline
%     Parameter & OECC & & \\
%     \hline
    
% \centering
% \end{tabular}
% \end{center}

